A link invariant with values in the Witt ring

Using Maslov indices, we show the existence of oriented link invariants with values in the Witt rings of certain fields. Various classical invariants are closely related to this construction. We also explore a surprising connection with the Weil representation. This version is identical to the one accepted for publication in Quantum Topology.

==> intro.tex <==
\section{Introduction}

The {\em braid group on~$n$ strands}~$\B_n$ is the group generated
by~$n-1$ generators~$\sigma_1, \ldots, \sigma_{n-1}$ subject to the
relations~$\sigma_i \sigma_j = \sigma_j \sigma_i$ for $|i - j|>2$, while 
%
$$ \sigma_i \sigma_{i+1} \sigma_i = \sigma_{i+1} \sigma_i
\sigma_{i+1} \, .   $$
%
The well-known interpretation of~$\B_n$ in terms of geometric braids
(see \cite{kassel}, Theorem~1.12) allows one to define the operation
of {\em closure} $\beta \mapsto \hat \beta $ ({\em loc.\ cit.},
\S2.2): here~$\beta \in\B_n$ and~$\hat \beta $ is an oriented link in
Euclidean~$3$-space. The celebrated theorem of Alexander ({\em loc.\
  cit.}, \S2.3) asserts that any oriented link in~$\R^3$ is isotopic
to one of the form~$\hat \beta $ for some~$\beta $ belonging to
some~$\B_n$.

This process defines an equivalence relation on the disjoint
union~$\coprod_{n\ge 2} \B_n$, according to which~$\beta \sim \gamma $
whenever the links~$\hat \beta $ and~$\hat \gamma $ are
isotopic. Markov's theorem ({\em loc.\ cit.}, \S2.5) describes this
relation explicitly. Here we shall state the result in the following
form: a map~$f= \coprod_{n\ge 2} f_n$ on the above disjoint union,
with values in any set~$E$, is constant on the equivalence classes if
and only if the two following properties are satisfied:

(i) each $f_n$ is invariant under conjugation, that
is~$f_n(\gamma^{-1} \beta \gamma ) = f_n (\beta )$ for all~$\beta,
\gamma \in \B_n$.

(ii) for all~$n\ge 2$ and all~$\beta \in \B_n$ one has~$f_{n+1}(\iota_n(\beta)
\sigma_n^{\pm 1}) = f_n(\beta )$, where~$\iota_n$ denotes the inclusion
of~$\B_n$ into~$\B_{n+1}$.

Such a map is usually called a {\em Markov function}. It follows that
the value of a Markov function on a braid~$\beta $ only depends on the
closure~$\hat \beta $, and in view of Alexander's theorem we see that
a Markov function gives an oriented link invariant (and conversely).

Because of condition (i), a traditional strategy in order to produce
Markov functions is to start with a collection of
representations~$\rho_n : \B_n \to GL(V_n)$, where~$V_n$ is a module
over some ring~$R$, and then rely on functions which are known to be
conjugation-invariant on the group of invertible matrices, like the
trace or determinant. A standard example is the Alexander-Conway
polynomial, which relies on the Burau representation and the
determinant ({\em loc.\ cit.}, \S3.4). Here~$R= \z[t, t^{-1}]$ and the
invariant takes its values in~$R$.

Our objective in this paper is to show that, given representations as
above with the extra property that~$\B_n$ preserves a symplectic or
anti-hermitian form, there is a natural conjugation-invariant
function~$f_n$ on~$\B_n$ with values in a Witt ring. The construction
of~$f_n$ is based on the Maslov index. It is easy to write down the
condition for the~$f_n$'s, taken together, to form a Markov function,
and we show that in the case of the Burau representation, they do. (So
far there seems to be no other example.) This affords new oriented
link invariants, with values in various Witt rings corresponding to
the various fields that one can decide to work on. 

More precisely, here are the contents of the paper. In Section 2, we
give some recollections on Witt rings and Maslov indices, and using
these we show that a representation of a braid group which preserves
an anti-hermitian form gives rise to a conjugation-invariant
function. In Section 3 we apply this machinery to the Burau
representation and obtain our main theorem (\ref{thm-main}). To give a
taste of this result now, let us state a particular case. 

\begin{thm} \label{thm-echantillon}
There is a unique Markov function~$(f_n)_{n\ge 2}$ with values in the
hermitian Witt ring~$\WH(\Q(t))$ of the field of rational fractions
in~$t$ over~$\Q$ satisfying the two properties below:
\begin{enumerate}
\item $f_n(\sigma_i) = 0$ for~$\sigma_i\in B_n$,
\item $f_n(\beta \gamma ) = f_n(\beta ) + f_n(\gamma ) +
  \maslov{\Gamma_1}{\Gamma_{r_n(\beta )}}{\Gamma_{r_n(\beta \gamma  )}}$.
\end{enumerate}
\end{thm}

Here~$r_n : \B_n \to GL_n(\Q(t))$ is the Burau representation, the
notation~$\Gamma_g$ is used for the graph of~$g$, and~$\tau$ is the
Maslov index, which takes three lagrangians as input and yields an
element in the Witt ring.

Link invariants ought to be easy to compute. Should the above theorem
appear too abstract, we urge the reader to refer to Section 4 where
concrete calculations are carried. We show that the above theorem
yields a Laurent-polynomial invariant akin to the Alexander-Conway
polynomial. We also exploit our method to produce a ``signature'' for
each complex number~$\omega $ of module~$1$, that is a~$\Z$-valued
invariant. When~$\omega$ is a root of unity, this invariant agrees
with the Levine-Tristram signature, as follows
from~\cite{ghys}. Indeed, the importance of this work by Gambaudo \&
Ghys cannot be overstated; it makes the first solid connection between
link invariants and the Maslov index, and inspired much of the present
paper. 


The Markov function in theorem~\ref{thm-echantillon}, among other
things, thus unifies the various signatures into a single link
invariant. It follows that two links which are distinguished by at
least one of these signatures are also distinguished by our Witt
invariant; for example there certainly exist links having the same
HOMFLY polynomial but different~$\omega$-signatures for some~$\omega$,
and our invariant must also take different values for these.

To emphasize how computable this invariant remains, we have made a
{\sc Sage} script available for download on the authors' webpages. It will
automatically perform all necessary calculations with the Markov
function.

Finally in Section 5 we relate our construction to the Weil
representation of the metaplectic group, and show that a certain
formula of Thomas (see \cite{thomas}) for the trace of this
representation actually yields a link invariant. This invariant can be
expressed in terms of the signature and the Alexander-Conway
polynomial, but the proof does use Maslov indices and ideas from the
previous sections. There is also a Weil representation over finite
fields, and a corresponding result which sheds light on the work of
Goldschmidt and Jones (see \cite{jones}).

In a subsequent paper it will be established that, at the price of
more machinery including a recent theorem of Barge and Lannes on
Maslov indices over rings, we can follow the above outline
over~$\z[\frac{1} {2}, t, t^{-1} ]$ instead of a field. There results
a single link invariant which specializes to all the others, thus
pushing the unification a step further. What is more, it will be shown
that our method extends to the case of {\em coloured links}, for which
the braid groups have to be replaced by an appropriate groupoid.

\noindent {\em Acknowledgments.} The authors wish to think \'Etienne
Ghys, Jean Barge, and Christian Kassel for their interest in the
paper. Our thanks extend to Hubert Rubenthaler for helpful discussions
on the harmonic analysis underlying the Weil representation. 

==> mathscommands.tex <==
\usepackage{amsmath, amssymb, amsfonts, amscd, amsthm}

%%%%%%%%%%%%%%  new commands %%%%%%%%%%%%%%%%%%%%
\newcommand{\maslov}[3]{\tau( #1,~#2,~#3    )}
\newcommand{\meyer}[2]{\maslov{\Gamma_1 }{\Gamma_{#1}} {\Gamma_{#2}}}

\newcommand{\Z}{\mathbb{Z}}
\newcommand{\C}{\mathbb{C}}
\newcommand{\R}{\mathbb{R}}
\newcommand{\Q}{\mathbb{Q}}
\newcommand{\F}{\mathbb{F}}


\newcommand{\z}{\mathbb{Z}}
\newcommand{\r}{\mathbb{R}}
\newcommand{\q}{\mathbb{Q}}
\newcommand{\f}{\mathbb{F}}



==> referee.tex <==
\section{Commentaires du referee}

Ghys and Gambaudo used the Burau representation and the Meyer co-cycle
for the symplectic group to relate the the signatures of the closures
of two braids to to the signature of the closure of their product.
Inspired by this result (and turning it around), Collinet and Guillot
have come up with a new way to define link invariants of Witt type
from the Burau representation and the Maslov index of Lagrangians
(interpreted as a Witt invariant).  They explore several examples of
this method and the resulting link invariants.  In the cases that they
analyze in any detail, the invariants seem to be determined by the the
Alexander-Conway polynomial and the signature function (on the unit
circle). However they point out many further invariants of Witt type
which they do not explore in detail.

I found this paper to be very interesting. It is also well written
except for section 5. Section 5 is on the relations with Weil
representation, and is really just a sketch of the idea without enough
detail or specific references to check its validity.

I think this paper is quote original and the results are appealing.

I have some specific comments. I list first the comments which have
mathematical content. Later I list the more stylistic comments.


MATHEMATICAL CONCERNS

page 12 paragraph -2

{\em signed determinant} : given a non-singular, hermitian~$n \times
n$-matrix~$A$ representing an element in the Witt ring, then~$D(A)=
(-1)^{n+1} \det(A)$.

I think to make a well-defined invariant of Witt classes in this way
one should define $D(A)= (-1)^{\frac {n(n-1)}{2}} \det(A)$. See MH
page 7 or for the Hermitian case page 42 of Notes on the Witt
Classification of Hermitian Innerproduct Spaces Over a Ring of
Algebraic Integers by Pierre E. Conner for instance.  This invariant
is usually called the discriminant. To see why $(-1)^{n+1} \det(A)$ will
not do, let A be the 4x4 matrix whose only non-zero entries are ones
on the antidiagonal.

page 12 paragraph -2 This happens to be the Alexander-Conway
polynomial of~$L$.

Have you checked whether in all your calculations (for other braids)
the image of the Alexander-Conway polynomial of~$L$ in $k^\times /
N(K^\times)$ agrees with $D( \Theta_{\Q(t)}(L))$?  Do you conjecture or
know whether this is true for all links?

page 14 paragraph -4 It is clear by construction that~$\hat s(\theta
)$ agrees with the~$e^{i \theta }$-signature of the link, presented in
\S~\ref{subsec-signatures}.

This is not clear to me. Why should it be this rather than
\[ \hat s(\theta ) = \lim_{\alpha \to \theta, \alpha < \theta }
s(\alpha ) \, .  \] or the average of the one sided limits or the
actual value of $s(\theta)$.  In general, the Levine-Tristram
signature is defined at all points on the unit circle.  You have
already noted that these agree with the signatures of section 4.1 at
roots of unity.  Anyway please be clearer about what happens at the
jumps, if you know.

page 15 paragraph -3
$$ T(f) = \int_{M_{2n}(\R)} f(g) T(g) dg \, .  $$

I am very confused about the two appearances of T( ) here. Does T denote the same thing in both places?

page 15 paragraph -2 In \cite{thomas}, Thomas gives a description of
the map~$\theta_n $, which we partially reproduce below.

How does Thomas denote this function?

page 16 paragraph 1 since the cohomological considerations of \S
\ref{subsec-conj-inv} guarantee that it lifts to a map~$\B_{2n} \to
M_{2n} (\R)$, one may wish to use~$\theta_n^{-1}$ in order to produce
a Markov function.

Somehow you must specify a particular lift before you can compose it
with $\theta_n^{-1}$.  Until you specify this lift I don't see how you
can prove the equation in corollary 5.3 as the left hand side is
defined ambiguously.

page 17 paragraph 6 This is precisely Theorem 2A in \cite{thomas},
when the notation is understood.

I could not put this together. See my earlier question about what lift of $r_{2n}(\beta)$ is taken.



STYLISTIC SUGGESTIONS


page 1 abstract Using Maslov indices, we show the existence of
oriented link invariant

should say an oriented link

page 3 paragraph -3 The sentence "We may easily construct the
map~$f_{2n} \colon B_{2n}\to \Z \cong W(\R)$ which appears in
Theorem~\ref{thm-example}"

should be explained. Something like: one does this by picking a
1-cochain for $B_n$ with co-boundary the 2 co-cycle for $B_n$ given by
$-\maslov{\Gamma_1}{\Gamma_{r_n(\beta )}}{\Gamma_{r_n(\beta \gamma )}}$

page 5 paragraph 4 (In other words, if this hermitian form is
degenerate, we consider the non-degenerate space obtained by an
appropriate quotient.)

would be better: More precisely, if this hermitian form is degenerate,
we take the non-degenerate space obtained by an appropriate quotient.

page 7 paragraph 8
In~$B_n$ there is an element~$\alpha $ such that~$\alpha \sigma_i
\alpha^{-1} = \sigma_{i+1}$ (for example~$\alpha = \sigma_1 \sigma_2
\cdots \sigma_{n-1}$)

This also used to establish equation (*) just above it. So it would be
better placed above equation (*)

page 9 paragraph 6

It us amusing to start with proving the existence of another Markov
function:

would be better: We first prove the the existence of another Markov
function which is used in the proof that $f_n$ is Markov.

page 10 in statement of Lemma 3.3 instead of $ \frac{1} {2} \dim U$
perhaps $\dim \ell_1$ would be better as it would make literally
correct the statement later on the same page: indeed going into a
larger braid group only adds a common summand to ALL the subspaces in
sight, which does not affect the equality of dimensions to be proved.

page 11 paragraph 5 For each oriented link~$L$, we obtain a set of
primes which is an invariant of~$L$, namely the set of those~$p$ for
which~$\Theta_\Q(L)$ maps to a non-zero element via the residue
map~$W(\Q) \to W(\F_p)$. Of course, for each~$p$ the value
in~$W(\F_p)$ is also an invariant.

This is repeated from the introduction. It should not be repeated here.

page 13 paragraph -1 (all real numbers but countably many will do) I
am not sure what you mean here


==> referee2.tex <==
Here are some modifications which we have made ``on our own'' (that
is, they were not prompted by your comments):


*** preliminary remark: we have changed §5.2, which started in the
    general case and ultimately used notation specific to K= R. Now
    for simplicity (and consistency!) it's written for K= R
    throughout. 

*** also, we have deleted the last few lines of §4, which are pretty
    much a repetition from the Introduction (I forget if this point
    was raised before and forgotten by all of us).


Now here are our answers to your queries (the obvious corrections have
been made and do not deserve comments here):


Q: page 14 middle of page
s(\theta) not explicitly defined anywhere.

A: We do write "This is a step function $s$" right before we write
$s(\theta)$ for the first time.







Q: page 12 line -3 This happens to be the Alexander-Conway polynomial
of $L$.  I take it that this only refers to L= the trefoil knot.  Or
are the authors claiming that this is true for all links L?  It should
be made clear what is claimed (and what is claimed should be proved.)
It would seem from their calculations posted on the web that the
authors have evidence either yeah or nay for the conjecture that
D( \Theta_{\Q(t)}(L)) is equal in k^\times / N(K^\times) to the image
of the Alexander-Conway polynomial.  It would be nice to know what the
experimental evidence says.


A: Originally we had only verified this on a few examples (where the
two polynomials were actually equal on the nose, not just in the
quotient group k^\times / N(K^\times). At your request, we have
systematically compared the two for all the knots considered on our
webpage (for general links (which may not be knots) the comparison
does not make sense, by the way, which somehow had discouraged us to
look into this closely): it turns out that they always agree! This is
now explained in §4.3.









Q: page 14 similar to the comments above on Alexander-Conway
polynomial: is it known (proved) how the Levine-Tristram signature
function compares to to the step functions s and \hat{s} defined on
this page? You do identify some the signatures in 4.1 with the values
of Levine-Tristram functions but these omega are algebraic and so
excluded from direct comparison.

A: At the moment, we cannot prove anything definite. However we hope
to prove that all the work we do in this paper can be performed over
Z[1/2, t, t^{-1}] rather than a field; this would remove the
restriction on theta and prove that the function s does indeed
computes the Levine-Tristram signature at least when theta is not a
``jump'' of s.











Q: page 17 line 6 the definition of the Weil character in Thomas
depends on the choice of an additive character \phi: R \rightarrow
C^x. Moreover the the Weil representation according to 2nd paragraph
of Thomas also depends of \phi. Thus the additvie character which
leads to the Weil character \gamma and the Weil rep rho in the present
paper should be specified.  Note that in page 112 of [LV] says that if
the additive character (denote chi rather than \phi in [LV]) is given
by \chi(x)=e^{2 i pi x}, then the Weil character \gamma(x) is given by
the complex conjugate of the formula given page 17 line 7 of this
paper.

A: Thanks for pointing this out. We use now the convention of
[LV]. See §5.3 and statement of Theorem 5.5.












Q: page 17 line -8 For Thomas tau( Gamma_g, Gamma_1, \ell oplus \ell)
is computed with respect to the form \bar{V} \oplus V, whereas in this
paper tau( Gamma_g, Gamma_1, \ell oplus \ell) is computed with respect
to the form V \oplus \bar{V}. Thus it seems to me in the statement of
Theorem 5.3 a conjugation should be placed over tau( Gamma_g, Gamma_1,
\ell oplus \ell) or equivalently an odd permutation should be
performed on the three lagrangians. But I believe 5.1 is correct as
stated using the form V \oplus \bar{V}.  Thus there then are some
needed changes in the statement of Theorem 5.5 which I leave to the
authors.


A: Again, thanks for spotting such a subtle mistake. After close
inspection, it turns out that 5.1 is *not* correct as stated, for the
following reason. Unsurprisingly, the little mistake is hidden in the
phrase ``after a minor rearrangement of the terms''. Indeed, this
involves replacing

T(L, aL, abL)

by

T(L + L, L + aL, L + abL)

(where T=\tau, L= \ell, +=\oplus). The idea is to appeal to the
additivity property (iii) of Maslov indices. However with our
definition of D(V) this should introduce a - sign...


So we have changed our definition of D(V) to that of
Thomas. Everything in §5 becomes true. Everything *else* is still true
without changes.

An issue for us is that our Sage script computes the opposite of
the invariant which we define in the paper... we've also had to change
the signs in our trefoil example.


==> sectiondefs.tex <==
\usepackage{titlesec}

% style des sections
\titleformat{\section}{\bf\center}{\S \arabic{section}.}{0.5em}{}
\titleformat{\subsection}[runin]{\bf}{\arabic{section}.\arabic{subsection}.}{.5em}{}[.]

==> thmdefs.tex <==
%%%%%%%%% theorems, definitions and shit %%%%%%%%%

%\swapnumbers

\newtheoremstyle{pedro}{}{}{\itshape}{}{\sc}{~--}{ }{\thmname{#1}\thmnumber{ #2}\thmnote{ (#3)}}

\newtheoremstyle{pedrodef}{}{}{}{}{\sc}{~--}{ }{\thmname{#1}\thmnumber{ #2}\thmnote{ (#3)}}


%%%%%%%%%% titre roman, texte italique %%%%%%%%%%%%%%%
\theoremstyle{pedro}
\newtheorem{lem}{Lemma}[section]
\newtheorem*{lem2}{Lemma}

\newtheorem{thm}[lem]{Theorem}
\newtheorem*{thm2}{Theorem}

\newtheorem{prop}[lem]{Proposition}
\newtheorem*{prop2}{Proposition}

\newtheorem{coro}[lem]{Corollary}
\newtheorem*{coro2}{Corollary}

\newtheorem{conj}[lem]{Conjecture}
\newtheorem*{conj2}{Conjecture}

%%%%%%%%% tout en italique %%%%%%%%%%%%%%%%%%%%%%%%%%%%
\theoremstyle{remark}
\newtheorem*{note2}{Note}
\newtheorem{rmk}[lem]{Remark}
\newtheorem*{rmk2}{Remark}
\newtheorem*{blank}{}

%%%%%%%%% tout en roman %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\theoremstyle{pedrodef}

\newtheorem{defn}{Definition}
\newtheorem{ex}[lem]{Example}
\newtheorem*{ex2}{Example}

